Neural Predicting Higher-order Patterns in Temporal Networks

Dynamic systems that consist of a set of interacting elements can be abstracted as temporal networks. Recently, higher-order patterns that involve multiple interacting nodes have been found crucial to indicate domain-specific laws of different temporal networks. This posts us the challenge of designing more sophisticated hypergraph models for these higher-order patterns and the associated new learning algorithms. Here, we propose the first model, named HIT, for full-spectrum higher-order pattern prediction in temporal hypergraphs. Particularly, we focus on predicting three types of common but important interaction patterns involving three interacting elements in temporal networks, which could be extended to even higher-order patterns. HIT extracts the structural representation of a node triplet of interest on the temporal hypergraph and uses it to tell what type of, when, and why the interaction expansion could happen in this triplet. HIT could achieve significant improvement (averaged 20% AUC gain to identify the interaction type, uniformly more accurate time estimation) compared to both heuristic and other neural-network-based baselines on 5 real-world large temporal hypergraphs. Moreover, HIT provides a certain degree of interpretability by identifying the most discriminatory structural features on the temporal hypergraphs for predicting different higher-order patterns.

==> 00-introduction-prev1.tex <==
\section{introduction}
 
 
Networks provide fundamental abstraction to study complex systems by viewing interacting elements as nodes and their interactions as links between nodes~\cite{newman2003structure}. Temporal networks track the interactions over time, which allows for more elaborate investigation of the dynamics of these systems~\cite{holme2012temporal,kovanen2011temporal}. How to model such dynamics to make inference over these networks has attracted much attention~\cite{snijders2010introduction,snijders2001statistical}. However, most works only focus on low-order patterns, \textit{e.g.}, link prediction between pairs of nodes~\cite{liben2007link,rahman2016link,zhu2016scalable,ma2017nonnegative,ma2018graph}. 


Many real-world systems consist of higher-order patterns that appear among more than two nodes and reflect much more complicated structures~\cite{benson2016higher,li2017inhomogeneous}: For example, in social networks, an individual can extend his/her social circles by being connected to another person, which contains only one pattern (Fig.~\ref{fig:illu} a). In contrast, when we investigate the social circle of a family with two people, it may be extended by adding one that either only one family member knows (Fig.~\ref{fig:illu} b) or both members know. The later case could be even more complicated, as it can be the case either the family members get to know the new one simultaneously (Fig.~\ref{fig:illu} d), say by inviting him/her to the family party, or via different social occasions (Fig.~\ref{fig:illu} c). To fully differentiate all the higher-order patterns, temporal links that happen in the same event should be formulated as a hyperedge (or a simplicial complex), which gives a hypergraph view of the network. Benson et al. studied the evolution of these patterns in the new view of both social and biological networks and confirmed their value of indicating domain-specific dynamics~\cite{benson2018simplicial}. %s are used to model high-order interactions that appear in a single even.   
Therefore, it is significant to build a model to predict higher-order patterns in hypergraphs, if one wants to learn the dynamics of different complex systems. A successful model may further benefit many group-targeted applications, such as group recommendation~\cite{amer2009group} or monitoring synergic actions of multiple genes~\cite{perez2009understanding}. 

%names these patterns as (b) wedge, (c) open triangle, (d) simplicial closure and

However, predicting higher-order patterns in temporal hypergraphs is challenging. To the best of our knowledge, no previous works can do so. The subtle difference among those patterns (Fig.~\ref{fig:illu} b-d) may need a model with strong representation power. Manually-design features are typically not enough. Heuristic metrics proposed for link prediction~\cite{liben2007link} have been generalized for higher-order link prediction in static networks~\cite{lahiri2007structure,benson2018simplicial,nassar2019pairwise,nassar2020neighborhood,yoon2020much}. Although the correlation between these heuristics and the higher-order patterns gets demonstrated~\cite{benson2018simplicial,yoon2020much}, the obtained performance marginally outperforms a random guessing baseline and is far from ideal to be used in practical systems.  

Neural networks due to their expressiveness have more potential to encode structural information~\cite{hamilton2017representation}. But higher-order dynamics entangles structural and temporal patterns and introduces additional challenges also for neural encoders. Recent works focused on predicting only specific higher-order patterns in either static networks~\cite{rossi2019higher,yadati2020nhp,cotta2020unsupervised,alsentzer2020subgraph}, or a few network snapshots~\cite{meng2018subgraph}.  %or single links in temporal networks~\cite{pareja2020evolvegcn,manessi2020dynamic,goyal2020dyngraph2vec,hajiramezanali2019variational,sankar2020dysat,trivedi2017know,trivedi2019dyrep,kumar2019predicting,xu2020inductive}. 
%Both  higher-order patterns with 
%Neither the full band of higher-order patterns nor elaborate temporal information get modelled properly. 
None of previous methods (either heuristic ones or neural networks) can be used to predict the entire spectrum of higher-order patterns (\textit{e.g.,} Fig.~\ref{fig:illu} b-d) let alone their evolution in the continuous time space. 

Here, we propose a novel neural network model, termed \textbf{HI}gher-order \textbf{T}emporal structure predictor (\proj) to predict higher-order network structures in continuous time space. For a proof of the concept, we focus on modeling the phenomenon of expending connection among three nodes as the patterns illustrated in Fig.~\ref{fig:illu}, also known as the procedure from an single link to a wedge, an open triangle or simplicial closure~\cite{benson2018simplicial}. The idea can be further generalized to learn more complicated patterns among more nodes. 

The key intuition of \proj is to properly encode the contextual temporal structure around three nodes of interest via neural networks and predict the future evolving patterns among them (Fig.~\ref{fig:model}). Because of the repetitive edges in temporal networks, the contextual structure could be much denser than static networks. Therefore, it is not scalable to digest the entire contextual structure and encode it via graph neural networks (GNN)~\cite{scarselli2008graph}. Instead, \proj samples and encodes a few {\em \underline{temporal random walks}} (TRW) to represent the structure. These TRWs start from those three nodes of interest and backtrack over time to collect structural and temporal features. Furthermore, to model the fundamental dynamics of each domain which is irrelevant node-personalized behaviors, \proj will remove node identities. This design guarantees good generalization of the model: The patterns extracted can be inductively applied across the network or even to other networks that share the similar dynamics. To compensate the loss of information by removing node identities, we generalize the {\em \underline{distance encoding}} technique (DE)~\cite{li2020distance} to encode each node that lies on the sampled temporal random walks. The original DE was used to improve the power of GNN to represent static networks. Our new DE is particularly designed for the temporal higher-order networks: Our DE is built upon the counts that one node appears at a certain position according to the set of sampled TRWs while leveraging a novel encoder to incorporate certain {\em asymmetry} to fit the higher-order patterns. Finally, \proj just needs to encode each DE-based TRW and then aggregate all TRWs to obtain the final representation for prediction. We conclude our contributions as the follows:

\begin{enumerate}[leftmargin=*]
    \item \proj is the first model to predict elaborated higher-order patterns in expanding connection from a single link to simplicial closure (Fig.~\ref{fig:illu} b-d). \proj achieves significant boost in predicting accuracy (xxx\%-xxx\% in AUC) compared to previous baselines that are used to predict some of these patterns.    
    \item \proj is the first model to predict higher-order network structures in continuous time space. \proj can also provide elaborate estimation of the time when different patterns in expanding connection may appear. 
    \item As \proj removes node identities and encodes TRW separately, it can automatically learn how different types of TRWs are most indicative to different higher-order patterns, which provide certain interpretation. We obtain the three data insights: 1) xxx 2) xxx 3) xxx.
\end{enumerate}







% Motivation: 
% \begin{itemize}
% \item From low-order to Higher-order study: Scope from traditional link prediction to higher-order structure prediction. Predict more complex higher-order behaviors: 1) For two people that are friends, will they get to know common friend in the future? Will they get to know the new friend in the same party or in two separate parties? When will they get to know this new friend? ... 

% \item Network dynamics methods: Improvetraditional basic statistic methods to neural methods --- Free from feature engineering: Does traditional metrics like common neighbors/A.A. scores/... still work in this much more complex cases? Can we even break these heuristics?

% \item Methodological contribution: Inspired by the distance encoding to model the correlation between more than 2 nodes. Our method can be viewed as a generalized version of the most recent casual anonymous work for pairwise nodes. 

% \item Insight contribution: Can we provide certain interpretation of our results?

% \end{itemize}

% Contributions:
% \begin{itemize}
% \item We are the first one to predict higher-order structures in dynamic graphs. Some works just considered predict higher-order structures in static graphs.

% \item Other dynamic network representation method can also be used for higher-order structure predictions. However, our neural methods are the ones that indeed capture the dynamics. Predict pairwise like -> simplicial complex closure, pairwise link prediction, wedge prediction... Predict accurate time.   

% \item Traditional scores: Common neighbors, xx, give pretty much random predictions, which kind of contradicts Benson's statement, as our problem is much more challenging. 

% \item Neural encoded features are indeed useful. Some two pieces insight from our interpretation results. We may expect our framework to help more domain scientists understand features.  
% \end{itemize}

==> 04-experiments_backup.tex <==


\begin{table*}[t]
\begin{minipage}{0.59\textwidth}
\small
\begin{center}
\scalebox{0.8}{
\begin{tabular}{c c c p{1.30cm}<{\centering} c c c }
\toprule  & \footnotesize{\# Node} & \footnotesize{\# Hyperedge} & \footnotesize{Ave. size}$^*$ & \footnotesize{\# Closure} & \footnotesize{\# Triangle} & \footnotesize{\#Wedge} \\
\midrule
tags-math-sx & 1.63K & 822K & 2.75 & 23.6K & 68.5K & 3.07M \\
tags-ask-ubuntu & 3.03K & 271K & 3.11 & 73.2K & 156K & 9.43M\\
congress-bills & 1.72K & 260K & 7.55 & 4.27M & 4.02M & 26.4M \\
DAWN & 2.56K & 2.27M & 2.59 & 45.8K & 62.3K & 3.13M \\
% NDC-substances & 5311 & 112K & 1.85 & 46.0K & 31.7K & 223K \\
threads-ask-ubuntu & 125K & 192K & 2.30 & 7.44K & 23.9K & 3.99M \\
% \# of Wedge & 3M & 9M & 3M & 26M & 223K \\
\bottomrule 
\end{tabular}
}
\end{center}

%\end{table}
\end{minipage}
\hfill
\scalebox{0.95}{
\begin{minipage}{0.40\textwidth}
\includegraphics[trim={0.3cm 0.4cm 0.5cm 0.7cm},clip,width=0.45\textwidth]{Figure_tags-ask-ubuntu.pdf}
\includegraphics[trim={0.3cm 0.4cm 0.5cm 0.7cm},clip,width=0.45\textwidth]{Figure_congress-bills.pdf}
%\caption{The distribution of time for the first pattern to appear(within $10\%T$ period) given $(\{u,v\},w,t)$}

\end{minipage}
}



% \vspace{-2mm}
\caption{\small{Basic statistics of the datasets. a) The numbers of different patterns in \{Wedge, Triangle, Closure\} within a time window $T_w = 0.1 * \text{the total time range}\,$ after initial interactions between the first two nodes get observed. *Ave. size is the averaged size of hyperedges. b) shows the distributions (PDF) of the times used to expand such interactions to the third nodes.}} %\pan{Add a) b) before the table and figures above; Enlarge the font in b); Draw histogram in b); Normalize the x-axis; Change the order of legends; Remove "time distribution of" from the figure title.}}
    \label{fig:data-stat}
    \vspace{-4mm}
\end{table*}


\begin{comment}
\begin{table*}[t]
\begin{minipage}{0.38\textwidth}
% \centering

% \includegraphics[trim={2.3cm 9.7cm 12.6cm 4.7cm},clip,width=1\textwidth, height=0.4\textwidth]{illu_new.pdf}
%     % \vspace{-2mm}
% \captionof{figure}{\small{Incremental processes of the interaction expansion among $\{u,v,w\}$}}
% % (lower order) or (b)-(d) from two nodes to a third node (higher order). Hypergraph modeling is needed to distinguish patterns (c) \textit{v.s.} (d): Starting from the initial hyperedge $\{u,v\}$, (c) has two hyperedges $\{u,w\},\{u,v\}$ while (d) has one single hyperedge $\{u,v,w\}$. }}
% \label{fig:illu}

\hfill

\includegraphics[trim={0.3cm 0.4cm 0.5cm 0.7cm},clip, %width=1\textwidth,
height=0.4\textwidth]{Figure_aa_t_tags-ask-ubuntu.pdf}

\hfill

\includegraphics[trim={0.3cm 0.4cm 0.5cm 0.7cm},clip, %width=1\textwidth,
height=0.4\textwidth]{Figure_aa_t_DAWN.pdf}

% \caption{Time distribution of tags-ask-ubuntu}
\captionof{figure}{\small{The distributions (PDF) of the arithmetic means of AA for three node pairs from $\{u,v,w\}$ under the time constraint $t$ over two datasets. \yunyu{Especially, if we want to learn what happened in a time window, we found these heuristic features of different phenomenon got severely entangled.
Figure~\ref{fig:aa_distribution} shows the AA distribution for four phenomenon. This indicates that heuristic features are not discriminant enough.  }
% \captionof{figure}{\small{The distributions (PDF) of the arithmetic means of AA's between $(u,v)$, $(u,w)$ and $(v,w)$ for triplets $(\{u,v\},w,t)$ over two datasets DAWN and tags-ask-ubuntu. 
% Distributions of different classes get severely mixed. 
}} \label{fig:aa_distribution}
\vfill
\end{minipage}
\begin{minipage}{0.59\textwidth}
% \begin{figure}
    \centering
    \includegraphics[trim={0.3cm 6.3cm 15.5cm 3.4cm},clip,width=1\textwidth]{data1.pdf}
        \vspace{-3mm}
    \captionof{figure}{\small{Prediction problems defined on temporal hypergraphs. After the first time $u, v$ interact, the questions focus on what type of, when and why such an interaction gets extended, \eg, to $w$.}}
    \label{fig:data-illu}
    % \vspace{-5mm}
% \end{figure}
\end{minipage}
\end{table*}
\end{comment}

% \vspace{-4mm}
\section{Experiments}
% \vspace{-2mm}
\label{sec:exp}

% \begin{textblock*}{1cm}(3.80cm,2.71cm) % {block width} (coords)
% %   \textbf{(a)}
%     \footnotesize{a)}
% \end{textblock*}
% \begin{textblock*}{1cm}(11.97cm,2.71cm) % {block width} (coords)
% %   \textbf{(b)}
%     \footnotesize{b)}
% \end{textblock*}

Here, we conduct an extensive evaluation of \proj to answer the three questions raised in Sec.\ref{sec:form}.
\textbf{Datasets.} We use five real-world temporal hypergraph datasets collected at~\cite{benson2018simplicial}: Tags-math-sx, Tags-ask-ubuntu, Congress-bills, DAWN, Threads-ask-ubuntu. Their detailed description is left in Appendix~\ref{sec:data}. The basic statistics of these datasets are shown in Table~\ref{fig:data-stat}. Note that repetitive temporal hyperedges significantly enlarge the network. %Although all the datasets have at most $5K$ nodes, the number of hyperedge starts from $112K$ to $2.27M$. 
Since the complexity is mainly dominated by the number of hyperedges (from $192K$ to $2.27M$), scalable models are needed. Moreover, the higher-order patterns can be extremely unbalanced. We also show the distributions of time used in interaction expanding for different patterns %in the right two figures of 
in Table~\ref{fig:data-stat} b). Triangles as expected take more time than Wedges while Closures unexpectedly share a similar tendency as Wedges.  


%The code of \proj is available \href{https://github.com/wenwen0319/HIT}{\emph{here}}. \yunyu{now it's my own github, remove this part before submission.}
%\vspace{-1mm}
%\subsection{Dataset}

% \begin{table*}
% \begin{center}
% \begin{tabular}{c c c c c c c c}

% \toprule  & tags-math-sx & tags-ask-ubuntu & DAWN & congress-bills & NDC-substances\\
% \midrule
% \# of Nodes & 1629 & 3029 & 2558 & 1718 & 5311\\
% \# of Hyperedges & 822059 & 271233 & 2272433 & 260851 & 112405\\
% Average Hyperedge Size & 2.19 & 2.71 & 1.58 & 3.66 & 1.85 \\
% \# of Closure & 23664 & 73202 & 45800 & 4270766 & 45993 \\
% \# of Triangle & 68477 & 156468 & 62308 & 4016648 & 31670 \\
% \# of Wedge & 3071242 & 9434139 & 3133513 & 26441913 & 223215 \\

% \bottomrule 

% \end{tabular}

% \end{center}
% \caption{$10\%$}
% \end{table*}

% \begin{table}
% \begin{center}
% \begin{tabular}{c c c c c c c c}

% \toprule  & tags-math-sx & tags-ask-ubuntu & DAWN & congress-bills & NDC-substances\\
% \midrule
% \# of Nodes & 1629 & 3029 & 2558 & 1718 & 5311\\
% \# of Hyperedges & 822K & 271K & 2M & 260K & 112K\\
% Average Hyperedge Size & 2.19 & 2.71 & 1.58 & 3.66 & 1.85 \\
% \# of Closure & 23K & 73K & 45K & 4M & 46K \\
% \# of Triangle & 68K & 156K & 62K & 4M & 31K \\
% \# of Wedge & 3M & 9M & 3M & 26M & 223K \\

% \bottomrule 

% \end{tabular}

% \end{center}
% \caption{$10\%$}
% \end{table}






%\yunyu{When checking the dataset, I found DAWN's time span is too small, about 32 different timestamps. So the time window }
%We use five temporal hypergraph datasets collected in~\cite{benson2018simplicial}. 
%\Reviewer{Also, the datasets are all pretty small in terms of the number of nodes. The
%scalability does not seem to be an issue, so experiments on larger datasets
%would be nice to have.}


%More detailed properties of these datasets are shown in Table~\ref{fig:data-stat}. \yunyu{Note that, we intentionally choose two similar datasets \textbf{tags-math-sx} and \textbf{tags-ask-ubuntu} to show our model is general. They should have similar performance since they have similar properties. } 
% Repetitive temporal hyperedges significantly enlarge the network\yunyu{. Although all the datasets have at most $5K$ nodes, the number of hyperedge starts from $112K$ to $2.27M$. Since the scalability is mainly dominated by the number of hyperedges, \sout{so}} scalable models are needed. Moreover, the higher-order patterns can be extremely unbalanced. We also show the distributions of time used in interaction expanding for different patterns in the right two figures. Triangles as expected take more time than Wedges while Closures unexpectedly share the similar tendency as Wedges.  


% tags-math-sx, tags-ask-ubuntu, DAWN, congress-bills, NDC-substances. Tags-math-sx and tags-ask-ubuntu are two collections of website Stack Exchange. Users can attach up to $5$ tags to each questions they post. We denote the tags as nodes. For each question, we connect all the corresponding tags. The timestamp is the time when the question was proposed. The Drug Abuse Warning Network (DAWN) records drug used by the patients. We denote the drugs as nodes. Each patient reports the drug they used before when they visit the emergency department. The timestamp is the time when the patients visit the emergency department. Congress-bills is the dataset of the bills from the sponsor and co-sponsors. These bills were put forth in the House of Representatives and the Senate. We denote the sponsors and co-sponsors as the nodes. The timestamp is the day when the bill were introduced. NDC-substances shows the relationship between the substances in different drugs. The nodes are the substances. The substances have connections if they belong to the same drug. The timestamps are the first day when the drug was marketed.

%\vspace{-1mm}
%\subsection{Data Preprocessing and Setup} \label{sec:preprocess}
%For each dataset, we order all the hyperedges by time. 
\textbf{Data Preprocessing and Setup.} Ideally, in temporal hypergraphs, hyperedges continue appearing over time but the datasets only include a certain time range $T$. To avoid the effect of the boundary truncation, we focus on all the node triplets between $[0.4T, 0.9T]$. We use the hyperedges in $[0T, 0.4T]$ to set up the initial network. Node triplets in $[0.4T, 0.75T]$ are selected for model training, $[0.75T, 0.825T]$ for validating and $[0.825T, 0.9T]$ for test. We also set the time window defined in Q1 as $T_w=0.1T$, so the hyperedges in $[0.9T, T]$ essentially complete the interaction expansion for the node triplets in the test set. We enumerate all the Edges, Wedges, Triangles, and Closures as the data instances with ground truth labels and properly balance all classes (see more details in Appendix~\ref{sec:proc}). %in training, validating, and test sets. 
%Since the data instances in different classes are extremely unbalanced (Table \ref{fig:data-stat}), we uniformly sample the same number of data instances from each class for training/evaluation/testing. The number of sampling instances are governed by the minimum size of the four classes. The sampled balanced dataset is shared cross different models. 
The performance of all methods is averaged across five-time independent experiments. %with the same random sampling process.
%We resample the data after each epoch.    
% the temporal networks within
%Consider the first $40\%$ of the time only contains little information, we will not sample the training, validating or testing set in the first $40\%$ edges.
%We choose all the edges appear after $40\%$ and before $75\%$ as the training set, all the edges appear after $75\%$ and before $82.5\%$ as the validating set and all the edges appear after $82.5\%$ and before $90\%$ as the testing set. We didn't use the last $10\%$ of edges because our time window is $10\%$ so we can not determine the patterns of the examples in the last $10\%$ edges. We enumerate all the close triangles, open triangles, wedges and no-new-edges in training, validating, and testing sets. Since the examples in different classes are unbalanced, for each epoch, we sample the same amount of examples from 4 patterns. And we resample the data after each epoch.

% For both tasks, we randomly pick $70\%$ of positive data and negative data as training set. Another $15\%$ of data as evaluation set. The final $15\%$ of data as the testing set. 

% We evaluate the confusion matrix and accuracy. 

%\vspace{-2mm}
%\subsection{Baselines}
%\Reviewer{It would be nice if there was some synthetic data under which the proposed
%performed proportional to some linear function of the distance encoding; in this
%case, can the proposed model learn the linear function (and do other methods
%still perform poorly)}

\textbf{Baselines.} To evaluate our method, we compare \proj with ten baseline methods, including both heuristic methods and NN-based encoders. The detailed description of them is left in the Appendix~\ref{sec:base}.

\vspace{-1mm}
\emph{Heuristic methods} are the metrics previously used for edge prediction~\cite{liben2007link} and recently got generalized for hyperedge prediction~\cite{benson2018simplicial,yoon2020much,nassar2020neighborhood}, including $3$-way Adamic Adar Index (\textbf{$3$-AA}), $3$-way Jaccard Coefficient (\textbf{$3$-JC}), $3$-way Preferential Attachment(\textbf{$3$-PA}), and the Arithmetic Mean of traditional \textbf{AA}, \textbf{JC} and \textbf{PA}.  %\pan{add other three, add references or explanation}. 
    %They were used in temporal hypergraphs for Triangle closure prediction. 
    Given a node triplet $(\{u,v\},w,t)$, we project hyperedges before $t$ into a static hypergraph, compute these metrics, and then impose a two-layer nonlinear neural network for prediction. %and report the best scores. %Detailed information can be found in the Appendix~\ref{sec:base}.
    % For AA, we compute the AA score for each node pair $(u,v)$, $(v,w)$, and $(u,w)$. %The obtained scores can be viewed as an embedding of the contextual structure of the node triplet. 
    % We try different combinations of these scores including using their Arithmetic means and
    % For the previous score, we imposed a two-layer neural network on them to make predictions and report their best results.
    % We apply the same procedure to PA and JC. For Arith., Geom., and Harm., we take the mean of the node degrees in the projected hypergraph and expand their dimensions via random Fourier features~\cite{rahimi2007random}. These features are fed into another two-layer neural network to make prediction.

% \emph{Heuristic methods} are the metrics previously used for edge prediction~\cite{liben2007link} and recently got generalized for hyperedge prediction~\cite{benson2018simplicial,yoon2020much,nassar2020neighborhood}, including Adamic Adar Index (\textbf{AA}), Preferential Attachment(\textbf{PA}), Jaccard Coefficient (\textbf{JC}), Arithmetic Mean (\textbf{Arith.}), Geometric Mean (\textbf{Geom.}), and Harmonic Mean (\textbf{Harm.}). %\pan{add other three, add references or explanation}. 
%     They were used in static hypergraphs and for only Closure prediction and we modify them properly to fit our setting. Given a node triplet $(\{u,v\},w,t)$, we project all the hyperedges before $t$ into a static hypergraph. For AA, we compute the AA score for each node pair $(u,v)$, $(v,w)$, and $(u,w)$. %The obtained scores can be viewed as an embedding of the contextual structure of the node triplet. 
%     We try different combinations of these scores including using their means and imposing a two-layer neural network on them to make predictions and report their best results. We apply the same procedure to PA and JC. For Arith., Geom., and Harm., we take the mean of the node degrees in the projected hypergraph and expand their dimensions via random Fourier features~\cite{rahimi2007random}. These features are fed into another two-layer neural network to make prediction.
    
   % Here the Arith., Geom., and Harm. are the arithmetic, geometric, and harmonic means of the degrees of the nodes.
    % \cite{benson2018simplicial,nassar2020neighborhood} to aggregate them into one score. 
    %The obtained scores can be viewed as an embedding of the contextual structure of the node triplet. Then, we use either random Fourier features~\cite{} or a two-layer nonlinear neural network to extend the dimension of this score for the final prediction. 
    %\yunyu{My current setting is directly sending three pairwise scores into a 2 layer nonlinear neural network.}
\vspace{-1mm}
 \emph{NN-based encoders} show great power in learning graph representations. However, none of the previous models can be directly applied to hyperedge prediction in temporal hypergraphs let alone the full spectrum of higher-order patterns.
 We adopt a hypergraph representation learning model \textbf{NHP}~\cite{yadati2020nhp} which is proposed for hyperedge prediction in static hypergraphs. For temporal hypergraphs, we aggregate hyperedges into 10 hypergraph snapshots. We train an \textbf{NHP} over these snapshots to get temporal node embeddings and then apply our decoders to make predictions. 
 We choose baselines \textbf{JODIE}~\cite{kumar2019predicting}, \textbf{TGAT}~\cite{xu2020inductive}, and \textbf{TGN}~\cite{tgn_icml_grl2020} as they are representatives models over temporal graphs. For a triplet $(\{u,v\},w,t)$, we use \textbf{JODIE}, \textbf{TGAT}, and \textbf{TGN} to generate node embeddings of $u,v,w$ and apply our decoders on these embeddings to make predictions. %Details on tuning these models are provided in the supplement.

%Six of them are heuristic metrics previously used for edge prediction~\cite{liben2007link} and recently generalized for hyperedge prediction~\cite{benson2018simplicial,yoon2020much}, including textbf{Adamic Adar Index(AA)}, \textbf{Preferential Attachment(PA)}, \textbf{Jaccard Coefficient(JC)}, \pan{add other three, add references or explanation}; The other three base 
%There are total five baselines, \textbf{Adamic Adar Index(AA)}, \textbf{Preferential Attachment(PA)}, \textbf{Jaccard Coefficient(JC)}, \textbf{JODIE}, and \textbf{TGAT}. Since no previous work focused on the triangle closure prediction problem, we choose three traditional methods and two deep learning methods as the baselines and do some modifications to them. For \textbf{AA}, \textbf{PA}, and \textbf{JC} three traditional features, given a triplet $(u,v,w)$ and the first edge among them $(e_{uv}^1, t_{uv}^1)$, we project all the edges before time $t_{uv}^1$ to the projected graph. Then we calculate \textbf{AA}, \textbf{PA}, and \textbf{JC} of each node pair $(u,v)$, $(v,w)$, and $(u,w)$. We use the average of three values as feature of the given triplet and first edge. After that the feature go through a two-layer nonlinear neural network to do the prediction. For \textbf{JODIE} and \textbf{TGAT}, both of them focused on the link prediction task. Here, we directly apply the same training process to get the node embedding. After that, we use the same classifier in the section~\ref{classifier} to get the final result. 

\begin{table*}[t]
\begin{center}

% \vspace{0.5cm}
\footnotesize
\begin{tabular}{c c c c c c c c}
\toprule ~  & \footnotesize{tags-math-sx} & \footnotesize{tags-ask-ubuntu}  & \footnotesize{congress-bills} & \footnotesize{DAWN} & \footnotesize{threads-ask-ubuntu}\\
\midrule
% JC & 67.23 $\pm$ 1.86 & 72.00 $\pm$ 0.17 & 61.81 $\pm$ 1.17 & 71.11 $\pm$ 1.57 & 54.87 $\pm$ 1.89\\
% PA & 67.52 $\pm$ 1.84 & 66.82 $\pm$ 1.24 & 60.78 $\pm$ 1.02 & 72.61 $\pm$ 1.58 & 57.84 $\pm$ 1.32\\
% AA & 75.80 $\pm$ 1.42 & 78.79 $\pm$ 1.09 & 77.11 $\pm$ 2.68 & 75.51 $\pm$ 1.21 & 57.38 $\pm$ 0.82\\

3-AA & 61.86 $\pm$ 0.25 & 68.31 $\pm$ 0.10 & 68.20 $\pm$ 0.21 & 72.75 $\pm$ 1.36 & 63.86 $\pm$ 0.16\\

3-JC & 58.62 $\pm$ 0.79 & 65.24 $\pm$ 0.18 & 69.22 $\pm$ 0.50 & 70.67 $\pm$ 0.59 & 63.59 $\pm$ 0.79\\

3-PA & 58.63 $\pm$ 0.79 & 55.96 $\pm$ 2.08 & 50.69 $\pm$ 0.62 & 51.48 $\pm$ 1.36 & 63.49 $\pm$ 1.49\\

AA & 65.05 $\pm$ 0.52 & 69.74 $\pm$ 0.28 & 70.22 $\pm$ 0.73 & 75.71 $\pm$ 0.36 & 76.52 $\pm$ 0.36 \\

% AA & 51.56 $\pm$ 0.28 & 53.02 $\pm$ 0.98 & 54.46 $\pm$ 1.08 & 52.20 $\pm$ 0.18 & 76.52 $\pm$ 0.36\\

JC & 60.76 $\pm$ 0.34 & 67.07 $\pm$ 0.11 & 68.24 $\pm$ 0.37 & 70.48 $\pm$ 0.63 & 68.84 $\pm$ 1.77\\

PA & 56.53 $\pm$ 2.04 & 65.71 $\pm$ 1.53 & 53.48 $\pm$ 3.19 & 65.60 $\pm$ 3.14 & 70.03 $\pm$ 1.10\\


% \midrule

NHP & 50.78 $\pm$ 0.29 & 51.42 $\pm$ 0.23 & 49.48 $\pm$ 0.12 & 49.90 $\pm$ 0.07 & 52.04 $\pm$ 0.79 \\

TGAT & 63.27 $\pm$ 0.27 & 53.75 $\pm$ 0.16 & 56.68 $\pm$ 0.22 & 46.63 $\pm$ 0.16 & 81.92 $\pm$ 0.25\\

JODIE & 56.68 $\pm$ 0.12 & 61.84 $\pm$ 0.48 & 63.50 $\pm$ 0.24 & 52.66 $\pm$ 0.27 & 67.23 $\pm$ 0.58 \\

TGN & 55.79 $\pm$ 0.16 & 54.33 $\pm$ 0.67 & 66.63 $\pm$ 0.23 & 71.84 $\pm$ 0.31 & 80.13 $\pm$ 0.79\\

% \midrule

\bf{\proj} & \bf{77.05 $\pm$ 0.31} & \bf{81.62 $\pm$ 0.69} & \bf{81.10 $\pm$ 0.26} & \bf{76.50 $\pm$ 0.79} & \bf{86.25 $\pm$ 0.15} \\

% \toprule  & \footnotesize{tags-math-sx} & \footnotesize{tags-ask-ubuntu} & \footnotesize{DAWN} & \footnotesize{congress-bills} & \footnotesize{NDC-substances}\\
% \midrule
% JC & 48.21 $\pm$ 0.06 & 46.78 $\pm$ 0.02 & 59.28 $\pm$ 0.01 & 46.56 $\pm$ 0.17 & 55.53 $\pm$ 0.05\\
% PA & 49.49 $\pm$ 0.09 & 48.68 $\pm$ 0.11 & 61.81 $\pm$ 0.15 & 49.51 $\pm$ 0.40 & 51.96 $\pm$ 0.29\\
% AA & 48.63 $\pm$ 0.27 & 46.64 $\pm$ 0.34 & 63.08 $\pm$ 0.36 & 48.74 $\pm$ 0.16 & 52.13 $\pm$ 0.82\\

% Arith. & 51.56 $\pm$ 0.28 & 53.02 $\pm$ 0.98 & 52.20 $\pm$ 0.18 & 54.46 $\pm$ 1.08 & 58.04 $\pm$ 0.21\\

% Geom. & 51.02 $\pm$ 0.06 & 50.77 $\pm$ 0.23 & 53.26 $\pm$ 0.53 & 61.84 $\pm$ 0.38 & 58.41 $\pm$ 0.13\\

% Harm. & 50.72 $\pm$ 0.22 & 48.19 $\pm$ 0.74 & 55.47 $\pm$ 1.12 & 64.90 $\pm$ 0.28 & 56.92 $\pm$ 0.24\\




% TGAT & 50.76 $\pm$ 0.26 & 53.75 $\pm$ 0.16 & 46.63 $\pm$ 0.16 & 56.68 $\pm$ 0.22 & 50.36 $\pm$ 0.57\\
% JODIE & 37.11 $\pm$ 0.30 & 61.84 $\pm$ 0.48 & 52.66 $\pm$ 0.27 & 63.50 $\pm$ 0.24 & 48.76 $\pm$ 0.26 \\
% NHP & 49.16 $\pm$ 0.21 & 47.45 $\pm$ 0.19 & 49.90 $\pm$ 0.07 & 49.48 $\pm$ 0.12 & 53.54 $\pm$ 0.26 \\
% \bf{\proj} & \bf{77.05 $\pm$ 0.31} & \bf{81.62 $\pm$ 0.69} & \bf{76.50 $\pm$ 0.79} & \bf{81.10 $\pm$ 0.26} & \bf{61.32 $\pm$ 0.60} \\

\bottomrule 

\end{tabular}

\end{center}
% \toprule \pan{Add 1 dataset}  & \footnotesize{tags-math-sx} & \footnotesize{tags-ask-ubuntu}  & \footnotesize{congress-bills} & \footnotesize{DAWN} & \footnotesize{NDC-substances}\\
% \midrule
% % JC & 67.23 $\pm$ 1.86 & 72.00 $\pm$ 0.17 & 61.81 $\pm$ 1.17 & 71.11 $\pm$ 1.57 & 54.87 $\pm$ 1.89\\
% % PA & 67.52 $\pm$ 1.84 & 66.82 $\pm$ 1.24 & 60.78 $\pm$ 1.02 & 72.61 $\pm$ 1.58 & 57.84 $\pm$ 1.32\\
% % AA & 75.80 $\pm$ 1.42 & 78.79 $\pm$ 1.09 & 77.11 $\pm$ 2.68 & 75.51 $\pm$ 1.21 & 57.38 $\pm$ 0.82\\

% 3-way AA & 61.86 $\pm$ 0.25 & 68.31 $\pm$ 0.10 & 68.20 $\pm$ 0.21 & 72.75 $\pm$ 1.36 & 59.62 $\pm$ 2.95\\

% 3-way JC & 58.62 $\pm$ 0.79 & 65.24 $\pm$ 0.18 & 69.22 $\pm$ 0.50 & 70.67 $\pm$ 0.59 & 59.31 $\pm$ 3.31\\

% 3-way PA & 58.63 $\pm$ 0.79 & 55.96 $\pm$ 2.08 & 50.69 $\pm$ 0.62 & 51.48 $\pm$ 1.36 & 53.49 $\pm$ 4.14\\

% Arith. of AA & 51.56 $\pm$ 0.28 & 53.02 $\pm$ 0.98 & 54.46 $\pm$ 1.08 & 52.20 $\pm$ 0.18 & 58.04 $\pm$ 0.21\\

% % Geom. of AA & 61.98 $\pm$ 0.30 & 69.51 $\pm$ 0.35 & 65.46 $\pm$ 0.84 & 74.34 $\pm$ 0.61 & 59.59 $\pm$ 3.22\\

% Arith. of JC & 60.76 $\pm$ 0.34 & 67.07 $\pm$ 0.11 & 68.24 $\pm$ 0.37 & 70.48 $\pm$ 0.63 & 54.60 $\pm$ 2.08\\

% Arith. of PA & 56.53 $\pm$ 2.04 & 65.71 $\pm$ 1.53 & 53.48 $\pm$ 3.19 & 65.60 $\pm$ 3.14 & 54.06 $\pm$ 3.24\\

% % Geom. of JC & 59.05 $\pm$ 0.45 & 65.04 $\pm$ 0.18 & 68.24 $\pm$ 0.37 & 70.48 $\pm$ 0.63 & 57.56 $\pm$ 2.59\\

% % Geom. of PA & 57.47 $\pm$ 1.42 & 63.55 $\pm$ 1.79 & 53.48 $\pm$ 3.19 & 65.60 $\pm$ 3.14 & 52.29 $\pm$ 1.14\\

% % Arith. & 51.56 $\pm$ 0.28 & 53.02 $\pm$ 0.98 & 54.46 $\pm$ 1.08 & 52.20 $\pm$ 0.18 & 58.04 $\pm$ 0.21\\

% % Geom. & 51.02 $\pm$ 0.06 & 50.77 $\pm$ 0.23 & 61.84 $\pm$ 0.38 & 53.26 $\pm$ 0.53 & 58.41 $\pm$ 0.13\\

% % Harm. & 50.72 $\pm$ 0.22 & 48.19 $\pm$ 0.74 & 64.90 $\pm$ 0.28 & 55.47 $\pm$ 1.12 & 56.92 $\pm$ 0.24\\




% TGAT & 50.76 $\pm$ 0.26 & 53.75 $\pm$ 0.16 & 56.68 $\pm$ 0.22 & 46.63 $\pm$ 0.16 & 50.36 $\pm$ 0.57\\
% JODIE & 37.11 $\pm$ 0.30 & 61.84 $\pm$ 0.48 & 63.50 $\pm$ 0.24 & 52.66 $\pm$ 0.27 & 48.76 $\pm$ 0.26 \\
% NHP & 49.16 $\pm$ 0.21 & 47.45 $\pm$ 0.19 & 49.48 $\pm$ 0.12 & 49.90 $\pm$ 0.07 & 53.54 $\pm$ 0.26 \\
% \bf{\proj} & \bf{77.05 $\pm$ 0.31} & \bf{81.62 $\pm$ 0.69} & \bf{81.10 $\pm$ 0.26} & \bf{76.50 $\pm$ 0.79} & \bf{61.32 $\pm$ 0.60} \\

% % \toprule  & \footnotesize{tags-math-sx} & \footnotesize{tags-ask-ubuntu} & \footnotesize{DAWN} & \footnotesize{congress-bills} & \footnotesize{NDC-substances}\\
% % \midrule
% % JC & 48.21 $\pm$ 0.06 & 46.78 $\pm$ 0.02 & 59.28 $\pm$ 0.01 & 46.56 $\pm$ 0.17 & 55.53 $\pm$ 0.05\\
% % PA & 49.49 $\pm$ 0.09 & 48.68 $\pm$ 0.11 & 61.81 $\pm$ 0.15 & 49.51 $\pm$ 0.40 & 51.96 $\pm$ 0.29\\
% % AA & 48.63 $\pm$ 0.27 & 46.64 $\pm$ 0.34 & 63.08 $\pm$ 0.36 & 48.74 $\pm$ 0.16 & 52.13 $\pm$ 0.82\\

% % Arith. & 51.56 $\pm$ 0.28 & 53.02 $\pm$ 0.98 & 52.20 $\pm$ 0.18 & 54.46 $\pm$ 1.08 & 58.04 $\pm$ 0.21\\

% % Geom. & 51.02 $\pm$ 0.06 & 50.77 $\pm$ 0.23 & 53.26 $\pm$ 0.53 & 61.84 $\pm$ 0.38 & 58.41 $\pm$ 0.13\\

% % Harm. & 50.72 $\pm$ 0.22 & 48.19 $\pm$ 0.74 & 55.47 $\pm$ 1.12 & 64.90 $\pm$ 0.28 & 56.92 $\pm$ 0.24\\




% % TGAT & 50.76 $\pm$ 0.26 & 53.75 $\pm$ 0.16 & 46.63 $\pm$ 0.16 & 56.68 $\pm$ 0.22 & 50.36 $\pm$ 0.57\\
% % JODIE & 37.11 $\pm$ 0.30 & 61.84 $\pm$ 0.48 & 52.66 $\pm$ 0.27 & 63.50 $\pm$ 0.24 & 48.76 $\pm$ 0.26 \\
% % NHP & 49.16 $\pm$ 0.21 & 47.45 $\pm$ 0.19 & 49.90 $\pm$ 0.07 & 49.48 $\pm$ 0.12 & 53.54 $\pm$ 0.26 \\
% % \bf{\proj} & \bf{77.05 $\pm$ 0.31} & \bf{81.62 $\pm$ 0.69} & \bf{76.50 $\pm$ 0.79} & \bf{81.10 $\pm$ 0.26} & \bf{61.32 $\pm$ 0.60} \\

% \bottomrule 

% \end{tabular}

% \end{center}
%\vspace{-4mm}

\vspace{-1mm}
\caption{\small{1-vs-1 AUC (mean$\pm$std) of higher-order pattern prediction (results for Q1): 1-vs-1 AUC is obtained by averaging AUCs of comparing the ground-truth class \text{v.s.} every other class in the multi-class classification.} %JC means Jaccord Coefficient. PA means Preferential Attachment. AA means Adamic Adar Index. Arith., Geom., and Harm. are the arithmetic, geometric, and harmonic means of the $3$ edge weights. We implement these $6$ traditional methods according to \cite{benson2018simplicial}. TGAT, JODIE are two Temporal Graph methods based on neural network. NHP is a Hypergraph method based on neural network.
}\label{tab:problem1_performance}
% \vspace{-6mm}
\end{table*}



%\Reviewer{The experiment is not that convincing. The first two datasets are similar and look redundant. The comparison methods are not state-of-the-art. Besides, the code is not available via the link in the paper. The pitfalls of the paper seems to be that the authors have not given proper justification as to why the baseline methods have poor performance in comparison to HIT on the evaluation tasks. Further, details are missing regarding the method to compute one-vs-one macro AUC.}

\vspace{-3mm}
\subsection{Predicting Higher-order Patterns (for Q1)}
% \vspace{-2mm}
% \begin{table*}[!ht]
% % \begin{minipage}{0.59\textwidth}
% \centering

% \includegraphics[trim={0.3cm 0.4cm 0.5cm 0.7cm},clip,width=0.49\textwidth]{Figure_tags-ask-ubuntu.pdf}
% \includegraphics[trim={0.3cm 0.4cm 0.5cm 0.7cm},clip,width=0.49\textwidth]{Figure_congress-bills.pdf}
% %\caption{The distribution of time for the first pattern to appear(within $10\%T$ period) given $(\{u,v\},w,t)$}


% \captionof{figure}{shows the distributions (PDF) of the times used to expand such interactions to the third nodes.}\label{fig:data-stat-2}
% % \end{minipage}
% \hfill

% % }%
% \vspace{-5mm}
% \centering
% % \caption{ pics}
% % \end{figure}
% \end{table*}


% \begin{minipage}{0.33\textwidth}
%   \centering
%     \includegraphics[trim={0.2cm 6.0cm 0.2cm 6.0cm},clip, scale=0.22]{Heatmap_tags-math-sx.pdf}
% %   \includegraphics[scale=0.32]{confusion_matrix_math.pdf}
% %   \caption{The confusion matrix of tags-math-sx, tags-ask-ubuntu, and congress-bills and the corresponding AUC score.}
% %   \label{fig:confusion_matrix}
% \end{minipage}
% \begin{minipage}{0.33\textwidth}
%   \centering
% %   \includegraphics[scale=0.32]{Figure_tags-ask-ubuntu_AUC.pdf}
%     \includegraphics[trim={0.2cm 6.0cm 0.2cm 6.0cm},clip, scale=0.22]{Heatmap_tags-ask-ubuntu.pdf}
% %   \caption{The confusion matrix of tags-math-sx, tags-ask-ubuntu, and congress-bills and the corresponding AUC score.}
% %   \label{fig:confusion_matrix}
% \end{minipage}
% \begin{minipage}{0.33\textwidth}
%   \centering
% %   \includegraphics[scale=0.32]{confusion_matrix_congress-bills.pdf}
%     \includegraphics[trim={0.2cm 6.0cm 0.2cm 6.0cm},clip, scale=0.22]{Heatmap_congress-bills.pdf}
% %   \caption{The confusion matrix of tags-math-sx, tags-ask-ubuntu, and congress-bills and the corresponding AUC score.}
% %   \label{fig:confusion_matrix}
% \end{minipage}



\begin{comment}

\begin{table}[t]
\begin{minipage}{0.43\textwidth}
\includegraphics[trim={0.3cm 0.4cm 0.5cm 0.7cm},clip,width=0.49\textwidth]{Figure_aa_t_tags-ask-ubuntu.pdf}
\includegraphics[trim={0.3cm 0.4cm 0.5cm 0.7cm},clip,width=0.49\textwidth]{Figure_aa_t_DAWN.pdf}

% \caption{Time distribution of tags-ask-ubuntu}
\captionof{figure}{\small{The distributions (PDF) of the arithmetic means of AA for three node pairs from $\{u,v,w\}$ under the time constraint $t$ over two datasets. %\yunyu{Especially, if we want to learn what happened in a time window, we found these heuristic features of different phenomenon got severely entangled.
%Figure~\ref{fig:aa_distribution} shows the AA distribution for four phenomenon. This indicates that heuristic features are not discriminant enough.  }
% \captionof{figure}{\small{The distributions (PDF) of the arithmetic means of AA's between $(u,v)$, $(u,w)$ and $(v,w)$ for triplets $(\{u,v\},w,t)$ over two datasets DAWN and tags-ask-ubuntu. 
% Distribusions of different classes get severely mixed. 
}} \label{fig:aa_distribution}
\end{minipage}
\hfill
\begin{minipage}{0.54\textwidth}
\small
\begin{center}
\begin{tabular}{c | c | c | c} 

\toprule  
\small{$\triangle$ AUC} & $\alpha = 0$ & \small{Rv. DE}  & \small{Sym. DE~\cite{li2020distance}} \\
\midrule
\small{tags-math-sx} & -10.05 & -14.28  & -9.53   \\
\small{tags-ask-ubuntu} & -5.98 & -14.03 & -8.23  \\ 


% Remove DE & 62.77 $\pm$ 0.31 & 67.59 $\pm$ 0.59 \\
% Remove TRW & 67.00 $\pm$ 0.37 & 75.64 $\pm$ 1.04 \\
% DE concat & 75.35 $\pm$ 0.49 & 81.07 $\pm$ 0.72\\
% Ours complete & 77.05 $\pm$ 0.31 & 81.62 $\pm$ 0.69  \\


\bottomrule 

\end{tabular}

\end{center}

\caption{\small{Ablation study (AUC). Revise each part of \proj and compare it with the full model in Table~\ref{tab:problem1_performance}. $\alpha=0$: Uniformly sample each step of TRWs. Rv. DE: Remove DEs (Eq.~\ref{eq:single-DE}). Sym. DE: Ignore asymmetry between DEs in Eq.~\eqref{eq:DE}. Aggregate three DEs via sum pooling~\cite{li2020distance}.}}\label{tab:ablation}

\end{minipage}
\vspace{-5mm}
\end{table}

\end{comment}







% \begin{table}[t]
% \small
% \begin{center}
% \begin{tabular}{c | c | c | c | c } 

% \toprule  
% \small{$\triangle$ AUC} & $\alpha = 0$ & \small{Removing DE}  & \small{Symmetric DE} & \small{Concat.} \\
% \midrule
% \small{tags-math-sx} & -10.05 & -14.28  & -9.53 & -0.7  \\
% \small{tags-ask-ubuntu} & -5.98 & -14.03 & -8.23 & -0.55  \\ 


% % Remove DE & 62.77 $\pm$ 0.31 & 67.59 $\pm$ 0.59 \\
% % Remove TRW & 67.00 $\pm$ 0.37 & 75.64 $\pm$ 1.04 \\
% % DE concat & 75.35 $\pm$ 0.49 & 81.07 $\pm$ 0.72\\
% % Ours complete & 77.05 $\pm$ 0.31 & 81.62 $\pm$ 0.69  \\


% \bottomrule 

% \end{tabular}

% \end{center}

% \caption{\small{Ablation study. We revise each part of \proj and compare the obtained performance (AUC) with the one for the full model in Table~\ref{tab:problem1_performance}. $\alpha=0$: We uniformly sample each step of TRWs. Removing DE: We remove DEs (Eq.~\ref{eq:single-DE}). Symmetric DE: We apply the same MLP over each DE in Eq.~\ref{eq:DE}. We ignore the asymmetry of patterns and aggregate them via sum pooling. Concat.: We ignore the symmetry of patterns and apply an MLP over the concatenation of  DEs in Eq.~\ref{eq:DE}.} }\label{tab:ablation}
% \end{table}


% \begin{table}[t]
% % \vspace{-15mm}
% \end{table}

%Identifying the type of patterns is a classification problem so we use the one-vs-one macro AUC value to evaluate the performance for all the baselines and our method. 
The results are shown in Table~\ref{tab:problem1_performance}. All baselines perform much worse than \proj, which confirms the need for more powerful models to extract subtle structural features to indicate higher-order patterns. % our statement that identifying dynamics inducing higher-order patterns is a challenging task and
%need more powerful models to extract the subtle structural features. 

As the training and test datasets are collected from the networks in different time ranges and do not share the exact same data distribution, some baseline approaches do not generalize well and achieve even less than 0.5 AUCs. %as the training and testing datasets do not share the exactly same data distribution, as they are collected from the networks in different time ranges. 
Previous works~\cite{benson2018simplicial,yoon2020much} demonstrate some possibilities of using heuristic metrics (AA, PA, JC) to distinguish Triangles and Closures in static hypergraphs. However, as shown in our results, these metrics fail to give desired predictions when time constraints are incorporated in the experimental setting. %We further investigate this observation by drawing the distributions of these metrics and indeed see that they get severely entangled across different classes (an example shown in Fig.~\ref{fig:aa_distribution}).
JODIE~\cite{kumar2019predicting} and TGN~\cite{tgn_icml_grl2020} do not work well because they track node embeddings over time which accumulate noise and do harm to transfer the knowledge of indicative patterns across different node triplets. TGAT~\cite{xu2020inductive} cannot distinguish nodes that have isomorphic contextual structures and thus fail to predict higher-order patterns. NHP~\cite{yadati2020nhp} uses network snapshots that lose much temporal information. A more detailed discussion on baselines is left in Appendix~\ref{sec:adv}.

% (an example shown in Fig.~\ref{fig:aa_distribution}). However, \proj achieves far better performance than all the baselines.


% \yunyu{Maybe a discussion of the results above here. Meanwhile, we suppose the baselines have poor performance for the following reasons. First, the overfiting problem could be observed for some baseline approaches when the training and testing datasets do not share the same data distribution, as they are collected from the networks in different time stamps. Secondly, for heuristic methods, they are not able to handle temporal information. In \cite{benson2018simplicial, yoon2020much}, they claimed the heuristic features are helpful. Interestingly, after we applied the time constraints, we found these metrics (AA, PA, JC) distributions are severely entangled as shown in Figure~\ref{fig:aa_distribution}. Consequently, these metrics are not able to generate stable predictions. Thirdly, for the NN based baselines, since there is no temporal hypergraph methods, we adopted the state-of-the-art models \textbf{JODIE} and \textbf{TGAT} from temporal network, and \textbf{NHP} from static hypergraphs respectively. For \textbf{JODIE} and \textbf{TGAT}, the clique expansion can be applied to transfer the hypergraph into a traditional graph. However, too much structural information is loss. Fourthly, for the static hypergraph approach \textbf{NHP}, we split the original hypergraphs into $10$ snapshots to handle the temporal information. This is also a common technique in traditional network. However, the performance is still poor. We suppose it is because the compressed snapshots impede the temporal information. By comparing all these baselines, it is obvious that our model performances the best and can handle the problem that the previous model cannot. }

% \sout{ The overfiting problem could be observed for some baseline approaches when the training and testing datasets do not share the same data distribution, as they are collected from the networks in different time stamps. Interestingly, previous works~\cite{benson2018simplicial,yoon2020much} demonstrate some possibilities of using heuristic metrics (AA, PA, JC) to distinguish Triangles and Closures in static hypergraphs. However, as shown in our results, these metrics often fail to generate stable predictions when time constraints are incorporated in the experimental setting. We further investigate this observation by drawing the distributions of these metrics and indeed see that they get severely entangled across different classes (an example shown in Fig.~\ref{fig:aa_distribution}).} However, \proj achieves far better performance than all the baselines. %though there is still some space for further improvement.


% \begin{wrapfigure}{R}{0.53\textwidth}
% \vspace{-6mm}
% \small

\begin{center}
\scalebox{0.9}{
\begin{tabular}{c | c | c | c  } 

\toprule  
\small{$\triangle$ AUC} & $\alpha = 0$ & \small{Rv. DE}  & \small{Sym. DE~\cite{li2020distance}} \\
\midrule
% \small{tags-math-sx} & -10.05 & -14.28  & -9.53   \\
% \small{tags-ask-ubuntu} & -5.98 & -14.03 & -8.23  \\ 
\footnotesize{tags-ask-ubuntu} & -1.59 & -4.42 & -3.13   \\
\footnotesize{threads-ask-ubuntu} & -2.16 & -3.44 & -2.68  \\ 


% Remove DE & 62.77 $\pm$ 0.31 & 67.59 $\pm$ 0.59 \\
% Remove TRW & 67.00 $\pm$ 0.37 & 75.64 $\pm$ 1.04 \\
% DE concat & 75.35 $\pm$ 0.49 & 81.07 $\pm$ 0.72\\
% Ours complete & 77.05 $\pm$ 0.31 & 81.62 $\pm$ 0.69  \\


\bottomrule 

\end{tabular}

}
\end{center}
% \vspace{-2mm}
\captionof{table}{\small{Ablation study (AUC). Revise each part of \proj and compare with the full model in Table~\ref{tab:problem1_performance}. $\alpha=0$: Uniformly sample each step of TRWs. Rv. DE: Remove DEs (Eq.~\ref{eq:single-DE}). Sym. DE: Ignore asymmetry between DEs in Eq.~\eqref{eq:DE}. Aggregate three DEs via sum pooling~\cite{li2020distance}.}}\label{tab:ablation}
% \vspace{-2mm}
% \end{wrapfigure}

To better interpret the results, we show the confusion matrices of \proj in Fig.~\ref{fig:confusion_matrix} for two networks, while the ones for the other two networks are left in Appendix~\ref{sec:confusion}. \proj identifies four patterns reasonably well in all these two datasets. Interestingly, \proj tends to incorrectly predict true Edges more as Triangles/Closures than as Wedges in the tag dataset. We see that in this dataset, triplets of interest share similar contextual structures are likely to either evolve to Triangles/Closures in a short time or avoid interaction expansion instead of keeping being Wedges. We also show some results of the ablation study of \proj in Table~\ref{tab:ablation}. We demonstrate the significance of time-based TRW sampling. Moreover, DEs that capture both the symmetry and asymmetry of the patterns perform much better than the sum pooling operation adopted in \cite{li2020distance}, which is crucial to distinguish the patterns such as Wedge \textit{v.s.} Triangle.

%while may confuse Triangles and Closure in congress-bills and threads-ask-ubuntu. 

\begin{comment}
To better interpret the results, we show the confusion matrices of \proj in Fig.~\ref{fig:confusion_matrix}. \proj identifies four patterns reasonably well in tags-ask-ubuntu and congress-bills, while may confuse Wedges and Triangles in tags-math-sx. Note that Wedges and Triangles are two strongly correlated patterns and a Wedge may evolve to a Triangle eventually. \proj captures the features that Wedges and Triangles share. Moreover, \proj tends to incorrectly predict true Edges more as Triangles/Closures than as Wedges in the two tags datasets. In these two datasets, triplets of interest share similar contextual structures are likely to either evolve to Triangles/Closures in a short time or avoid interaction expansion instead of keeping being Wedges. The results of the ablation study of \proj are shown in Table~\ref{tab:ablation}. We demonstrate the significance of time-based TRW sampling. Moreover, DEs that capture both the symmetry and asymmetry of the patterns perform much better than the sum pooling operation adopted in \cite{li2020distance}.  
\end{comment}
 %The result illustrates that both DE and TRW contribute a significant performance improvement while the DE concat has a comparable result with our complete. We believe it is because our pipeline is powerful enough to learn the structral and temporal information.

%This is counter-intuitive due to the hierarchy between these patterns.
%the classification result of class $1$(Open Triangles) and class $3$(No-new-edges) is worse than class $2$(Wedges) and class $3$(No-new-edges). This is counter-intuitive since the adjacent classes should be more similar according to our definition. We conjecture that open triangles and no-new-edges have more similarities than wedge and no-new-edges. A triplet with no-new-edges are more likely to transform into an open triangle instead of a wedge.

%The predefined a time window for Question 1 may introduce some confusing patterns.



%Being collected at different time ranges, the training and testing datasets do not share extractly the same data distribution, so some  

%need a extremely powerful model to extract the subtle difference in the structural features. 
%fail to classify $4$ classes and their performance are just slightly better than random guessing. For the traditional baselines(JC, PA, AA), the performance shows that the traditional static graph features cannot capture the triplet information. For deep-learning based link-prediction methods, although they can handle the link prediction tasks, they fail to capture the information among a triplet. The main reason is that most link prediction task ignore the time information(\eg, JODIE, TGAT). Therefore, the embedding from these models does not contain the time information and therefore they can not distinguish close and open triangles or if there will be a triangle closure in a time window.  In our triangle prediction task, two node pairs with relative distance do not provide enough information. Compared with the baselines, our method has a significantly better performance. 


%\subsection{Results and discussions}
% \begin{figure}[t]

    


% relative or COMPARATIVE? 
% Meanwhile, most link prediction methods are designed based on the relative relation between two node pairs instead of the exact value of each node pair. Due to the testing configuration of most link prediction models(\ie, we sample the same amount of positive and negative samples and calculate the score. Then, we choose the top $50\%$ as there will be a link in the future), this will not effect 

%\subsection{Confusion Matrix}

% The confusion matrix aims to analyze which class our model can distinguish most. Here, we show the confusion matrix of training, validating and testing set of tags-math-sx to show the details of our model.


% From three confusion matrices, we can find that under most circumstances, the training, testing and validating sets have a similar distribution. This proves that our model is not overfitting or underfitting. Besides, there are a few interesting findings. First, our model is more likely to consider the triplet as class $0$(Close Triangles) and class $1$(Open Triangles). Because in a temporal network, all node pairs will eventually have connections as the time goes by. We believe our model captures the similarly property. Secondly, the classification result of class $1$(Open Triangles) and class $3$(No-new-edges) is worse than class $2$(Wedges) and class $3$(No-new-edges). This is counter-intuitive since the adjacent classes should be more similar according to our definition. We conjecture that open triangles and no-new-edges have more similarities than wedge and no-new-edges. A triplet with no-new-edges are more likely to transform into an open triangle instead of a wedge.

% train acc: 0.5053337696335078, val acc: 0.5128585446859903, test acc: 0.5101029116465864
% 2021-01-05 08:50:53,531 - root - INFO - train auc: 0.7542304096080514, val auc: 0.7704365287527035, test auc: 0.7715336673194996
% 2021-01-05 08:50:53,531 - root - INFO - train ap: 1.0, val ap: 1.0, test ap: 1.0
% 2021-01-05 08:50:54,979 - root - INFO - start 9 epoch
% 2021-01-05 09:31:34,008 - root - INFO - confusion matrix: 
% 2021-01-05 09:31:34,008 - root - INFO - [7862 3100 1610 2696 2134 6741 3601 2792 1887 4880 6559 1942 1708 2123
%  1537 9900]
% 2021-01-05 09:45:47,273 - root - INFO - confusion matrix: 
% 2021-01-05 09:45:47,273 - root - INFO - [2919  580  383  533  876 1741 1061  737  770 1423 1771  451  806  797
%   238 2574]
% 2021-01-05 09:59:39,054 - root - INFO - confusion matrix: 
% 2021-01-05 09:59:39,055 - root - INFO - [2586  543  362  490  768 1661  979  573  670 1244 1676  391  907  654
%   120 2300]

% \begin{figure*}[t]
%  %\includegraphics[trim={1cm 6.0cm 1cm 6.0cm},clip, width=0.245\textwidth]{Heatmap_tags-math-sx.pdf}
%  \includegraphics[trim={1cm 6.0cm 1cm 6.0cm},clip, width=0.25\textwidth]{Heatmap_tags-ask-ubuntu.pdf}
%  \includegraphics[trim={1cm 6.0cm 1cm 6.0cm},clip, width=0.25\textwidth]{Heatmap_congress-bills.pdf}
%  \includegraphics[trim={1cm 6.0cm 1cm 6.0cm},clip, width=0.25\textwidth]{Heatmap_threads-ask-ubuntu.pdf}
%  \vspace{-6mm}
% \caption{\small{The confusion matrices of \proj to make prediction over tags-ask-ubuntu, congress-bills and threads-ask-ubuntu and the corresponding AUC scores.} }
% \label{fig:confusion_matrix}
% \vspace{-5mm}
% \end{figure*}

\vspace{-5mm}
\begin{figure}[htbp]
\centering
 %\includegraphics[trim={1cm 6.0cm 1cm 6.0cm},clip, width=0.245\textwidth]{Heatmap_tags-math-sx.pdf}

 \includegraphics[trim={1cm 5.8cm 1cm 6.0cm},clip, width=0.195\textwidth]{Heatmap_tags-ask-ubuntu.pdf}
%  \includegraphics[trim={1cm 6.0cm 1cm 6.0cm},clip, width=0.25\textwidth]{Heatmap_congress-bills.pdf}
 \hspace{1mm}
 \includegraphics[trim={1cm 6.0cm 1cm 6.0cm},clip, width=0.2\textwidth]{Heatmap_threads-ask-ubuntu.pdf}
 \vspace{-6mm}

\caption{\small{The confusion matrices of \proj to make prediction over tags-ask-ubuntu and threads-ask-ubuntu and the corresponding AUC scores.} }
\label{fig:confusion_matrix}
\vspace{-5mm}
\end{figure}


% \begin{wrapfigure}{R}{0.53\textwidth}

%\begin{minipage}{0.55\textwidth}
% \vspace{-12mm}
\begin{center}
\scalebox{0.75}{
\begin{tabular}{ c | c c c | c c c  } 

\toprule  
\multicolumn{1}{c|}{ ~ } & 
% & & 
\multicolumn{3}{c|}{tags-math-sx} & \multicolumn{3}{c}{tags-ask-ubuntu}  \\
\cline{2-7}
\multicolumn{1}{c|}{ ~ }  & \footnotesize{Wedge} & \footnotesize{Triangle} & \footnotesize{Closure} & \footnotesize{Wedge} & \footnotesize{Triangle} & \footnotesize{Closure} \\
\midrule
% NLL
% & Closure & Triangle & Edge & Closure & Triangle & Edge & Closure & Triangle & Edge & Closure & Triangle & Edge & Closure & Triangle & Edge
% \\
% \midrule
% JC & & & & & \\
% PA & & & & & \\
% AA & & & & & \\
%\multirow{5}*{\footnotesize{NLL}}&

\footnotesize{TGAT} & 1.54 & 0.77 & 1.37 & 1.55 & 1.03 & 1.40  \\

\footnotesize{JODIE} & 1.47 & 2.60 & 2.71 & 1.91 & 0.94 & 1.36 \\

% ~&\footnotesize{NHP} & 1.07 & 0.61 & 1.30 & 1.47 & 0.84 & 1.35  \\

\footnotesize{TGN} & 1.23 & 0.69 & 1.45 & 1.50 & 0.87 & 1.37  \\

\footnotesize{\textbf{\proj}} & 1.21 & 0.61 & 1.19 & 1.33 & 0.84 & 1.34 
\\
% \midrule
% MSE
% & Closure & Triangle & Edge & Closure & Triangle & Edge & Closure & Triangle & Edge & Closure & Triangle & Edge & Closure & Triangle & Edge
% \\
%& \multicolumn{3}{|c|}{tags-math-sx} & \multicolumn{3}{|c|}{tags-ask-ubuntu} & \multicolumn{3}{|c|}{DAWN} & \multicolumn{3}{|c|}{congress-bills} & \multicolumn{3}{|c|}{NDC-substances} \\
% \midrule
% JC & & & & & \\
% PA & & & & & \\
% AA & & & & & \\
% ~&
% \footnotesize{TGAT} & 0.17 & 0.07 & 0.18 & 0.17 & 0.09 & 0.15  \\

% \footnotesize{MSE}&\footnotesize{JODIE} & 0.16 & 0.15 & 0.22 & 0.18 & 0.08 & 0.15  \\

% \footnotesize{-LOG} &\footnotesize{NHP} & XX & XX & XX & XX & XX & XX   \\

% ~ &\footnotesize{TGN} & XX & XX & XX & XX & XX & XX   \\

% ~&\footnotesize{\textbf{\proj}} & 0.18 & 0.07 & 0.12 & 0.15 & 0.08 & 0.16 
%  \\


\bottomrule 

\end{tabular}
}
\end{center}
% \vspace{-2mm}
\captionof{table}{\small{Averaged NLL (Eq.~\eqref{eq:NLL}) of time prediction (for Q2): Lower is better. %\pan{Some results are need to be redone. Moreover, we need a full evaluation on all 5 datasets (perhaps, in the supplement).
}}\label{tab:time_prediction_performance}
%\captionof{table}{\small{NLL (Eq.~\eqref{eq:NLL}) of time prediction (for Question 2): Lower is better. MSE-LOG: $(\log t-\hat{\log t})^2$ where $\log t$, $\hat{\log t}$ are the ground-truth and the estimated log time, respectively.}}\label{tab:time_prediction_performance}
\vspace{-3mm}
%\end{minipage}
% \end{wrapfigure}


\vspace{-2mm}
\subsection{Time Prediction (for Q2)}
\vspace{-1mm}


\proj can predict when a triplet of interest expands the interaction into a certain higher-order pattern for the first time. In this study, we only compare our method with NN-based baselines except NHP because heuristic baselines are found not expressive enough to capture elaborate temporal information, and NHP uses network snapshots and cannot be applied. All the baselines share the same maximum-likelihood decoder for Q2 as \proj defined in Sec.~\ref{sec:decoder}. We use NLL (Eq.\eqref{eq:NLL}) as the evaluating metrics, which is superior in evaluating how different models leanr the underlying distributions of the time. %We use the expectation of the learnt Gaussian mixture as the estimation of log time. %MSE-LOG provides an explication charaterization of the gap between this estimated log time and the ground truth. %
%MSE-LOG  
We report the results in Table~\ref{tab:time_prediction_performance} (complete results on all datasets can be found in Appendix~\ref{sec:full-time-est}). \proj estimates the distributions of the time uniformly more accurately than baselines.
%\proj achieves much more accurate estimation than baselines. %By analyzing MSE-LOG, with some simple algebra, \proj is expected to yield a time estimation $\hat{t}\in[1.4^{-1}t, 1.4t]$ where $t$ is the ground truth. In contrast, baselines yields a estimation in $[3.3^{-1}t, 3.3t]$ and \proj reduces the approximation factor of the estimation by about 60\%.   

% \begin{textblock*}{1cm}(1.55cm,3.07cm) % {block width} (coords)
%   \textbf{(a)}
% \end{textblock*}
% \begin{textblock*}{1cm}(11.85cm,3.07cm) % {block width} (coords)
%   \textbf{(b)}
% \end{textblock*}

% \textbf{AA}
% \textbf{JC}
% \textbf{JODIE} DAWN, congress-bills $64$ embedding dimension. Others $128$ embedding dimension
% \textbf{TGAT}

% \begin{table}[t]

% \begin{center}

% % \vspace{0.5cm}
% \scalebox{0.5}{  
% \begin{tabular}{c c c c }

% \toprule Tasks (AUC) & Closure \textit{v.s.} Triangle (65.63) & Closure and Triangle \textit{v.s.} Wedge (57.58) & Wedge \textit{v.s.} Edge (71.10)\\
% \midrule
% \multirow{2}*{Largest $C_W$} & \textcolor[RGB]{34, 139, 34}{(\{$x$, $x$\}, 0) (\{1, $x$\}, 1) (\{$x$, $x$\}, 2)} $100.00\%$ & (\{0, $x$\}, $x$) (\{1, $x$\}, $x$) (\{2, $x$\}, 1) $84.26\%$ & (\{$x$, 0\}, $x$) (\{$x$, 1\}, $x$) (\{$x$, 2\}, 2) $49.14\%$ \\
% ~ & \textcolor{blue}{(\{0, $x$\}, $x$) (\{1, $x$\}, 1) (\{2, $x$\}, $x$)} $100.00\%$ & (\{0, $x$\}, $x$) (\{1, $x$\}, $x$) (\{2, $x$\}, 2) $66.13\%$ & (\{$x$, 0\}, $x$) (\{$x$, 1\}, $x$) (\{$x$, 2\}, $x$) $50.26\%$ 
% \\
% % ~ & \bf{(\{0, $x$\}, $x$) (\{1, $x$\}, 2) (\{2, $x$\}, $x$)} $92.36\%$ & (\{$x$, $x$\}, 0) (\{$x$, $x$\}, 1) (\{2, $x$\}, 2) $66.73\%$ & (\{0, $x$\}, $x$) (\{1, 2\}, $x$) (\{2, $x$\}, $x$) $26.21\%$\\
% \midrule
% \multirow{2}*{Smallest $C_W$} & (\{0, $x$\}, $x$) (\{1, $x$\}, $x$) (\{1, $x$\}, $x$) $38.94\%$ & \textcolor{blue}{(\{0, $x$\}, $x$) (\{1, $x$\}, $x$) (\{1, $x$\}, $x$)} $34.68\%$ & \textcolor{blue}{(\{$x$, 0\}, $x$) (\{$x$, 1\}, $x$) (\{1, 2\}, $x$)} $24.60\%$
% \\
% ~ & (\{0, $x$\}, $x$) (\{1, $x$\}, $x$) (\{2, 2\}, $x$) $54.49\%$  & \textcolor[RGB]{34, 139, 34}{(\{$x$, 0\}, $x$) (\{$x$, 1\}, $x$) (\{$x$, 2\}, $x$)} $49.74\%$ & \textcolor[RGB]{34, 139, 34}{(\{$x$, 0\}, $x$) (\{$x$, 1\}, $x$) (\{2, 2\}, $x$)} $28.81\%$

   
% \\
% % ~ & (\{$x$, $x$\}, 0) (\{2, $x$\}, 1) (\{$x$, $x$\}, 2) $93.94\%$ & \bf{(\{$x$, $x$\}, 0) (\{$x$, $x$\}, 1) (\{$x$, $x$\}, 2)} $49.88\%$ & \bf{(\{0, $x$\}, $x$) (\{1, $x$\}, $x$) (\{2, 2\}, $x$)} $52.69\%$
% % \\
% \bottomrule 

% \end{tabular}
% }
% \end{center}

% \caption{\small{The TRWs with the top-2 largest and smallest scores $C_W$ (Eq.~\eqref{eq:TRW-score}) to distinguish two patterns in tags-ask-ubuntu. TRWs are categorized based on DEs: Given a node triplet $(\{u,v\},w,t)$, a TRW $W$ is categorized based on $W = (I(W[0]),I(W[1]),I(W[2]))$ where $I(a)=(\{\tilde{g}(a;S_u),\tilde{g}(a;S_v)\},\tilde{g}(a;S_w))$, $\tilde{g}(a;S_z)$ uses SPD (Eq.\eqref{eq:spd}) and $x$ indicates SPD$\geq3$. \proj uses %these TRWs and 
% the decoder for Q3. The ratio besides each TRW refers the number of the corresponding TRWs that appear as features for the first class over that for both classes. }}\label{tab:interpretation} 
% \vspace{-6mm}
% \end{table}
\begin{figure*}
% \centering
 \begin{minipage}{0.25\textwidth}
% \begin{table}
% \begin{center}
% \vspace{0.5cm}
\scalebox{0.48}{  
\begin{tabular}{c c c c }

\toprule Tasks (AUC) & Closure \textit{v.s.} Triangle (65.63) & Closure and Triangle \textit{v.s.} Wedge (57.58) & Wedge \textit{v.s.} Edge (71.10)\\
\midrule
\multirow{2}*{Largest $C_W$} & \textcolor[RGB]{34, 139, 34}{(\{$x$, $x$\}, 0) (\{1, $x$\}, 1) (\{$x$, $x$\}, 2)} $100.00\%$ & (\{0, $x$\}, $x$) (\{1, $x$\}, $x$) (\{2, $x$\}, 1) $84.26\%$ & (\{$x$, 0\}, $x$) (\{$x$, 1\}, $x$) (\{$x$, 2\}, 2) $49.14\%$ \\
~ & \textcolor{blue}{(\{0, $x$\}, $x$) (\{1, $x$\}, 1) (\{2, $x$\}, $x$)} $100.00\%$ & (\{0, $x$\}, $x$) (\{1, $x$\}, $x$) (\{2, $x$\}, 2) $66.13\%$ & (\{$x$, 0\}, $x$) (\{$x$, 1\}, $x$) (\{$x$, 2\}, $x$) $50.26\%$ 
\\
% ~ & \bf{(\{0, $x$\}, $x$) (\{1, $x$\}, 2) (\{2, $x$\}, $x$)} $92.36\%$ & (\{$x$, $x$\}, 0) (\{$x$, $x$\}, 1) (\{2, $x$\}, 2) $66.73\%$ & (\{0, $x$\}, $x$) (\{1, 2\}, $x$) (\{2, $x$\}, $x$) $26.21\%$\\
\midrule
\multirow{2}*{Smallest $C_W$} & (\{0, $x$\}, $x$) (\{1, $x$\}, $x$) (\{1, $x$\}, $x$) $38.94\%$ & \textcolor{blue}{(\{0, $x$\}, $x$) (\{1, $x$\}, $x$) (\{1, $x$\}, $x$)} $34.68\%$ & \textcolor{blue}{(\{$x$, 0\}, $x$) (\{$x$, 1\}, $x$) (\{1, 2\}, $x$)} $24.60\%$
\\
~ & (\{0, $x$\}, $x$) (\{1, $x$\}, $x$) (\{2, 2\}, $x$) $54.49\%$  & \textcolor[RGB]{34, 139, 34}{(\{$x$, 0\}, $x$) (\{$x$, 1\}, $x$) (\{$x$, 2\}, $x$)} $49.74\%$ & \textcolor[RGB]{34, 139, 34}{(\{$x$, 0\}, $x$) (\{$x$, 1\}, $x$) (\{2, 2\}, $x$)} $28.81\%$

   
\\
% ~ & (\{$x$, $x$\}, 0) (\{2, $x$\}, 1) (\{$x$, $x$\}, 2) $93.94\%$ & \bf{(\{$x$, $x$\}, 0) (\{$x$, $x$\}, 1) (\{$x$, $x$\}, 2)} $49.88\%$ & \bf{(\{0, $x$\}, $x$) (\{1, $x$\}, $x$) (\{2, 2\}, $x$)} $52.69\%$
% \\
\bottomrule 

\end{tabular}
}
% \end{center}

% \caption{\small{The TRWs with the top-2 largest and smallest scores $C_W$ (Eq.~\eqref{eq:TRW-score}) to distinguish two patterns in tags-ask-ubuntu. TRWs are categorized based on DEs: Given a node triplet $(\{u,v\},w,t)$, a TRW $W$ is categorized based on $W = (I(W[0]),I(W[1]),I(W[2]))$ where $I(a)=(\{\tilde{g}(a;S_u),\tilde{g}(a;S_v)\},\tilde{g}(a;S_w))$, $\tilde{g}(a;S_z)$ uses SPD (Eq.\eqref{eq:spd}) and $x$ indicates SPD$\geq3$. \proj uses %these TRWs and 
% the decoder for Q3. The ratio besides each TRW refers the number of the corresponding TRWs that appear as features for the first class over that for both classes. }}\label{tab:interpretation} 
% \vspace{-6mm}
% \end{table}
\end{minipage}
\hfill
\begin{minipage}{0.25\textwidth}
% \begin{figure}[t]
 %\includegraphics[trim={1cm 6.0cm 1cm 6.0cm},clip, width=0.245\textwidth]{Heatmap_tags-math-sx.pdf}
 \includegraphics[trim={10.2cm 8.0cm 10cm 7.0cm},clip, width=0.3\textwidth]{inter-illu-1.pdf}
 
 \includegraphics[trim={10.0cm 8.7cm 10.3cm 6.9cm},clip, width=0.3\textwidth]{inter-illu-2.pdf}
 
 \includegraphics[trim={10.3cm 7.9cm 10cm 7.0cm},clip, width=0.3\textwidth]{inter-illu-3.pdf}
%  \vspace{-6mm}
% \caption{\small{Illustration of TRWs based on those \textcolor{blue}{blue} or \textcolor[RGB]{34, 139, 34}{green} TRWs in Table.~\ref{tab:interpretation}.} }
% \label{fig:inter-illu}
% \vspace{-5mm}
% \end{figure}
\end{minipage}
\captionof{figure}{\small{The above table is the TRWs with the top-2 largest and smallest scores $C_W$ (Eq.~\eqref{eq:TRW-score}) to distinguish two patterns in tags-ask-ubuntu. TRWs are categorized based on DEs: Given a node triplet $(\{u,v\},w,t)$, a TRW $W$ is categorized based on $W = (I(W[0]),I(W[1]),I(W[2]))$ where $I(a)=(\{\tilde{g}(a;S_u),\tilde{g}(a;S_v)\},\tilde{g}(a;S_w))$, $\tilde{g}(a;S_z)$ uses SPD (Eq.\eqref{eq:spd}) and $x$ indicates SPD$\geq3$. \proj uses the decoder for Q3. The ratio besides each TRW refers the number of the corresponding TRWs that appear as features for the first class over that for both classes. The bottom figures are th illustration of TRWs based on those \textcolor{blue}{blue} or \textcolor[RGB]{34, 139, 34}{green} TRWs in the above table.
% Figure.~\ref{tab:interpretation}. 
}} \label{tab:interpretation} 
\end{figure*}

\begin{textblock*}{1cm}(2.30cm,2.71cm) % {block width} (coords)
%   \textbf{(a)}
    \footnotesize{a)}
\end{textblock*}
\begin{textblock*}{1cm}(12.40cm,2.71cm) % {block width} (coords)
%   \textbf{(b)}
    \footnotesize{b)}
\end{textblock*}

% \vspace{-3mm}
\subsection{Most Discriminatory TRWs (for Q3)}
% \vspace{-2mm}
Searching for the important features that induce certain prediction is always a challenging problem in machine learning, especially for NN-based models. Identifying network structural features is even more challenging as they are irregular and strongly correlated by nature. %Although still not ideal, 
\proj provides possibilities to identify the most discriminatory structural features in the format of TRWs. As illustrated in Sec.\ref{sec:decoder} decoder for Q3, \proj allows categorizing TRWs into different types and summarized the impact of each individual type as a single score from the higher-order pattern prediction. 

We evaluate \proj over tags-ask-ubuntu.
%For a more meaningful feature and a better visualization, we use TRWs with SPD as DEs (Eq.~\eqref{eq:spd}) and train \proj to classify two selected higher-order patterns in tags-ask-ubuntu. 
We rank different types of TRWs based on their discriminatory scores $C_W$ (Eq.\eqref{eq:TRW-score}) and list the top-2 ranked TRWs in Table~\ref{tab:interpretation}. Because the NN-based encoder encodes each TRW separately to achieve $C_W$ and the decoder is simply a linear logistic regression, \proj yields very stable model interpretations. The top-2 ranked TRWs always stay in the top-5 ranked ones in the five random experiments.

We further sample $3,000$ examples for each classification task and compute the ratio of each type of TRWs that appear as the features for the first class and both two classes (first + second). We see a good correlation between the discriminatory score $C_W$'s and the ratios, which indicates the effectiveness of \proj in selecting indicative TRW features.
%Note that those ratios can hardly be used as the discriminatory scores as they do not consider the correlation between different types of TRWs, while $C_W$'s can as they are obtained via training. 

Those most discriminatory TRW features shown in Table~\ref{tab:interpretation} demonstrates interesting patterns. We further study these patterns by using three examples as illustrated in 
Fig.~\ref{tab:interpretation}
% Fig.~\ref{fig:inter-illu} 
%\yunyu{Fig.~\ref{tab:interpretation}}
(TRWs with blue or green font in 
the table 
% Table~\ref{tab:interpretation}
are drawn). Consider a node triplet $(\{u,v\},w,t)$. 

% \begin{wrapfigure}{r}{0.2\textwidth}
% \begin{minipage}{1\textwidth}
% \begin{figure}
%   \centering
% \vspace{-10mm}
%   \includegraphics[trim={9.8cm 4.5cm 10.5cm 2.45cm}, clip, width=0.2\textwidth ]{inter-illu.pdf}
%  \vspace{-6mm}
% \captionof{figure}{\small{Illustration of TRWs based on those \textcolor{blue}{blue} or \textcolor[RGB]{34, 139, 34}{green} TRWs in Table.~\ref{tab:interpretation}.} %The green and blue lines indicates to TRWs indicating the corresponding classification task. } 
%   }
% \label{fig:inter-illu}
% \vspace{-5mm}
% \end{figure}
% \end{minipage}
% \end{wrapfigure}

% \begin{figure}[t]
%  %\includegraphics[trim={1cm 6.0cm 1cm 6.0cm},clip, width=0.245\textwidth]{Heatmap_tags-math-sx.pdf}
%  \includegraphics[trim={10cm 8.0cm 10cm 7.0cm},clip, width=0.15\textwidth]{inter-illu-1.pdf}
%  \includegraphics[trim={10cm 8.7cm 10cm 6.9cm},clip, width=0.15\textwidth]{inter-illu-2.pdf}
%  \includegraphics[trim={10cm 7.9cm 10cm 7.0cm},clip, width=0.15\textwidth]{inter-illu-3.pdf}
% %  \vspace{-6mm}
% \caption{\small{Illustration of TRWs based on those \textcolor{blue}{blue} or \textcolor[RGB]{34, 139, 34}{green} TRWs in Table.~\ref{tab:interpretation}.} }
% \label{fig:inter-illu}
% \vspace{-5mm}
% \end{figure}

\textbf{TRWs that indicate Closures as opposed to Triangles}: They start from $u,v$ (or $w$) and jump to some nodes that are directly connected to $w$ (or $u,v$). This means that $u,v,w$ tend to form a Closure pattern if both $u,w$ and $v,w$ have common neighbors before. We may interpret it as a higher-order pattern closure that generalizes triadic closure in graphs~\cite{simmel1950sociology}. Without hypergraph modeling, we cannot distinguish Closures and Triangles, and thus cannot observe this higher-order pattern closure.
    
\textbf{TRWs that indicate Wedges as opposed to Closures + Triangles}: They start from $u$ (or $v$, $w$) and jump to some nodes that are still far away from the other two nodes. These TRWs can be viewed as the opposite of the above higher-order pattern closure. An interesting question is whether they are the most indicative ones for Edges. See the next bullet. 

\textbf{TRWs that indicate Edges as opposed to Wedges}: Interestingly, they follow a uniform pattern by jumping around $u$ and $v$. Therefore, the most indicative features that forbid any interaction expansion are the structures that densely connect $u$ and $v$ but disconnect $w$. On the other hand, combined with the previous bullet, the most indicative features for interaction expansion but from only one node (Wedges) are the structures that connect a single node in the node triplet.

% \begin{itemize} [leftmargin=*]
%     \item TRWs that indicate Closures as opposed to Triangles: They start from $u,v$ (or $w$) and jump to some nodes that are directly connected to $w$ (or $u,v$). This means that $u,v,w$ tend to form a Closure pattern if both $u,w$ and $v,w$ have common neighbors before. We may interpret it as a higher-order pattern closure which generalizes triadic closure in simple graphs~\cite{simmel1950sociology}. Without hypergraph modeling, we cannot distinguish Closures and Triangles, and thus cannot observe this higher-order pattern closure.
    
%     \item TRWs that indicate Wedges as opposed to Closures + Triangles: They start from $u$ (or $v$, $w$) and jump to some nodes that are still far away from the other two nodes. These TRWs can be viewed as the opposite of the above higher-order pattern closure. An interesting question is whether they are the most indicative ones for Edges. See the next bullet. 
%     \item TRWs that indicate Edges as opposed to Wedges: Interestingly, they follow a uniform pattern by jumping around $u$ and $v$. Therefore, the most indicative features that forbid any interaction expansion are the structures that densely connect $u$ and $v$ but disconnect $w$. On the other hand, combined with the previous bullet, the most indicative features for interaction expansion but from only one node (Wedges) are the structures that connect a single node in the node triplet.
% \end{itemize}
%In our paper, we try to capture the motifs in the temporal network by the Causal Random Walk and Set-based Anonymization. Considered the motifs are crucial in temporal networks, here we do further study to learn the interpretation of different motifs. There are so many different motifs in a network. Our aim is to find out which patterns are the most important patterns.


%To learn the motifs, we divided the Causal Random Walks according to the encoding $g(\omega, S_i)$. If the nodes $\omega$ in two walks $\tilde{W_1}$ and $\tilde{W_2}$ have the same encoding $g(\omega, S_i)$, where $i \in \{u,v,w\}$, then we consider these two walks have the same pattern. Considered that the original $g(\omega, S_i)$ contains too much patterns, we modify our model a little bit. We change the $g(\omega,S_i)$ to the shortest path distance. That is, $g(\omega, S_i)$ is the shortest path distance between $\omega$ and $S_i$. We denote the original $g(\omega, S_i)$ as $g_{lp}$, and the shortest path distance as $g_{spd}$. For $g_{lp}$, it is strictly powerful than $g_{spd}$. This is because we can consider the first position of $\omega$ appears in the $g_{lp}$ as the shortest path distance. Our performance also shows that compared with $g_{lp}$, $g_{spd}$ has a lower performance. 

 



% \begin{table}[t]
% \small
% \begin{center}
% \begin{tabular}{c | c | c } 

% \toprule  

% & \footnotesize{tags-math-sx} & \footnotesize{tags-ask-ubuntu} \\
% \midrule

% Remove DE & 62.77 $\pm$ 0.31 & 67.59 $\pm$ 0.59 \\
% Remove TRW & 67.00 $\pm$ 0.37 & 75.64 $\pm$ 1.04 \\
% DE concat & 75.35 $\pm$ 0.49 & 81.07 $\pm$ 0.72\\
% Ours complete & 77.05 $\pm$ 0.31 & 81.62 $\pm$ 0.69  \\


% \bottomrule 

% \end{tabular}

% \end{center}

% \caption{Ablation study. We remove each part of our model and conduct the same experiments. Remove DE means removing the whole distance encoding part. Remove TRW means we sample the walk uniformly without using the temporal information. DE concat means we directly concatenate in \eqref{eq:DE}, we directly concatenate $g(z;S_u)$, $g(z;S_v)$, and $g(z;S_w)$ and apply a neural network to extract the features. The result illustrates that both DE and TRW contribute a significant performance improvement while the DE concat has a comparable result with our complete. We believe it is because our pipeline is powerful enough to learn the structral and temporal information. }\label{tab:ablation}
% \vspace{-7mm}
% \end{table}


% \begin{table*}

% \begin{center}

% % \vspace{0.5cm}

% \begin{tabular}{c c c c }

% \toprule  & Closure \textit{v.s.} Triangle & Closure and Triangle \textit{v.s.} Wedge & Wedge \textit{v.s.} Edge\\
% \midrule
% \multirow{3}*{First Class} & (\{$\infty$, $\infty$\}, 0) (\{1, $\infty$\}, 1) (\{$\infty$, $\infty$\}, 2) & (\{0, $\infty$\}, $\infty$) (\{1, $\infty$\}, $\infty$) (\{2, $\infty$\}, 2) & (\{$\infty$, 0\}, $\infty$) (\{$\infty$, 1\}, $\infty$) (\{$\infty$, 2\}, 2) \\
% ~ & (\{0, $\infty$\}, $\infty$) (\{1, $\infty$\}, 1) (\{2, $\infty$\}, $\infty$) & (\{0, $\infty$\}, $\infty$) (\{1, $\infty$\}, $\infty$) (\{2, $\infty$\}, 1) & (\{$\infty$, 0\}, $\infty$) (\{$\infty$, 1\}, $\infty$) (\{$\infty$, 2\}, $\infty$) 
% \\
% ~ & (\{0, $\infty$\}, $\infty$) (\{1, $\infty$\}, 2) (\{2, $\infty$\}, $\infty$) & (\{$\infty$, $\infty$\}, 0) (\{$\infty$, $\infty$\}, 1) (\{2, $\infty$\}, 2) & (\{0, $\infty$\}, $\infty$) (\{1, 2\}, $\infty$) (\{2, $\infty$\}, $\infty$)\\
% \midrule
% \multirow{3}*{Second Class} & (\{0, $\infty$\}, $\infty$) (\{1, $\infty$\}, $\infty$) (\{2, 2\}, $\infty$) & (\{$\infty$, $\infty$\}, 0) (\{$\infty$, $\infty$\}, 1) (\{$\infty$, $\infty$\}, 2) & (\{$\infty$, 0\}, $\infty$) (\{$\infty$, 1\}, $\infty$) (\{1, 2\}, $\infty$)
% \\
% ~ & (\{0, $\infty$\}, $\infty$) (\{1, $\infty$\}, $\infty$) (\{1, $\infty$\}, $\infty$) & (\{$\infty$, 0\}, $\infty$) (\{$\infty$, 1\}, $\infty$) (\{$\infty$, 2\}, $\infty$) & (\{$\infty$, 0\}, $\infty$) (\{$\infty$, 1\}, $\infty$) (\{2, 2\}, $\infty$)

   
% \\
% ~ & (\{$\infty$, $\infty$\}, 0) (\{2, $\infty$\}, 1) (\{$\infty$, $\infty$\}, 2) & (\{0, $\infty$\}, $\infty$) (\{1, $\infty$\}, $\infty$) (\{1, $\infty$\}, $\infty$) & (\{0, $\infty$\}, $\infty$) (\{1, $\infty$\}, $\infty$) (\{2, 2\}, $\infty$)
% \\
% \bottomrule 

% \end{tabular}

% \end{center}

% \caption{Interpretation of different walks}\label{tab:interpretation}

% \end{table*}

% \newpage
% \pan{In this section, we will introduce dataset, preprocessing, baselines. For the results, we will provide two prediction tasks time-window-based prediction, time prediction. We also introduce interpretation results. }  

% \pan{We need to show: 1) A table to show the datasets: \# hyperedges, \# nodes, average hyperedge size, \# Closure, \#Triangle, \# wedge; 2) Draw the time distribution of all these three (10\% time window? or entire ?); 3) A table to compare the AUC. Show a table on detailed classes AUC of one best data set for baselines; 4) Pick another three datasets to draw the confusing matrix of our method; 5) Draw confusing distribution of heuristic scores; 6) A table to show time estimation (NLL and abs difference); 7) Any visualization for time estimation? ; 8) Interpretation tables (top 3 for each pair comparison). }

% \yunyu{2.1: 1, 2, 4, 5 2.2: 3, 6, 7, 8}

% \pan{1. Table transpose into one column version, digit accuracy; 2. Overlap the distribution (pdf) for two datasets and insert the figures; 3. Fill in all the baselines (AUC); Make the table into a minipage; AA scores for ubuntu and DAWN in a figure (put in the right of the minipage) 4. Keep math, ubuntu, congress in a line (Auc -> AUC); 6. Fill in the time estimation table (MSE), remove heuristic baselines; 7. Distribution figure with baselines (for the two datasets used in 2.; last step); 8. Plug in the table (pick one piece of insight for each classification task). Plug in the ratio of event-per-case. After this, we do another interpretation exp for congress-bill. 9. We also need some ablation study (vs no DE, symmetric DE, our DE, without time).}


    
% \begin{table*}[!ht]

% \begin{center}

% % \vspace{0.5cm}

% \begin{tabular}{c c c c }

% \toprule Tasks (AUC) & Closure \textit{v.s.} Triangle (65.63) & Closure and Triangle \textit{v.s.} Wedge (57.58) & Wedge \textit{v.s.} Edge (71.10)\\
% \midrule
% \multirow{3}*{Largest $C_W$} & \bf{(\{$x$, $x$\}, 0) (\{1, $x$\}, 1) (\{$x$, $x$\}, 2)} $100.00\%$ & (\{0, $x$\}, $x$) (\{1, $x$\}, $x$) (\{2, $x$\}, 1) $84.26\%$ & (\{$x$, 0\}, $x$) (\{$x$, 1\}, $x$) (\{$x$, 2\}, 2) $49.14\%$ \\
% ~ & \bf{(\{0, $x$\}, $x$) (\{1, $x$\}, 1) (\{2, $x$\}, $x$)} $100.00\%$ & (\{0, $x$\}, $x$) (\{1, $x$\}, $x$) (\{2, $x$\}, 2) $66.13\%$ & (\{$x$, 0\}, $x$) (\{$x$, 1\}, $x$) (\{$x$, 2\}, $x$) $50.26\%$ 
% \\
% ~ & \bf{(\{0, $x$\}, $x$) (\{1, $x$\}, 2) (\{2, $x$\}, $x$)} $92.36\%$ & (\{$x$, $x$\}, 0) (\{$x$, $x$\}, 1) (\{2, $x$\}, 2) $66.73\%$ & (\{0, $x$\}, $x$) (\{1, 2\}, $x$) (\{2, $x$\}, $x$) $26.21\%$\\
% \midrule
% \multirow{3}*{Smallest $C_W$} & (\{0, $x$\}, $x$) (\{1, $x$\}, $x$) (\{1, $x$\}, $x$) $38.94\%$ & \bf{(\{0, $x$\}, $x$) (\{1, $x$\}, $x$) (\{1, $x$\}, $x$)} $34.68\%$ & \bf{(\{$x$, 0\}, $x$) (\{$x$, 1\}, $x$) (\{1, 2\}, $x$)} $24.60\%$
% \\
% ~ & (\{0, $x$\}, $x$) (\{1, $x$\}, $x$) (\{2, 2\}, $x$) $54.49\%$  & \bf{(\{$x$, 0\}, $x$) (\{$x$, 1\}, $x$) (\{$x$, 2\}, $x$)} $49.74\%$ & \bf{(\{$x$, 0\}, $x$) (\{$x$, 1\}, $x$) (\{2, 2\}, $x$)} $28.81\%$

   
% \\
% ~ & (\{$x$, $x$\}, 0) (\{2, $x$\}, 1) (\{$x$, $x$\}, 2) $93.94\%$ & \bf{(\{$x$, $x$\}, 0) (\{$x$, $x$\}, 1) (\{$x$, $x$\}, 2)} $49.88\%$ & \bf{(\{0, $x$\}, $x$) (\{1, $x$\}, $x$) (\{2, 2\}, $x$)} $52.69\%$
% \\
% \bottomrule 

% \end{tabular}

% \end{center}

% \caption{\small{TRWs with the top-3 largest and smallest scores $C_W$ (Eq.~\eqref{eq:TRW-score}) to distinguish two patterns in tags-ask-ubuntu. TRWs are categorized based on DEs: Given a node triplet $(\{u,v\},w,t)$, a TRW $W$ is categorized based on $W = I(W[0])\,I(W[1])\,I(W[2])$ where $I(a)=(\{\tilde{g}(a;S_u),\tilde{g}(a;S_v)\},\tilde{g}(a;S_w))$, where $\tilde{g}(a;S_z)$ uses SPD (Eq.\eqref{eq:spd}) and $x$ indicates SPD$\geq3$. \yunyu{The ratio means the number of walks in the first class over all the number of all the walks.} \proj uses these TRWs and the decoder in Sec.~\ref{sec:decoder-3}.}}\label{tab:interpretation}

% \end{table*}


% \begin{tabular}{c c}

% \toprule Tasks (AUC) & Closure \textit{v.s.} Triangle (65.63) \\
% \midrule
% \multirow{2}*{Largest $C_W$} & \bf{(\{$x$, $x$\}, 0) (\{1, $x$\}, 1) (\{$x$, $x$\}, 2)} $100.00\%$   \\
% ~ & \bf{(\{0, $x$\}, $x$) (\{1, $x$\}, 1) (\{2, $x$\}, $x$)} $100.00\%$ \\
% % ~ & \bf{(\{0, $x$\}, $x$) (\{1, $x$\}, 2) (\{2, $x$\}, $x$)} $92.36\%$ & (\{$x$, $x$\}, 0) (\{$x$, $x$\}, 1) (\{2, $x$\}, 2) $66.73\%$ & (\{0, $x$\}, $x$) (\{1, 2\}, $x$) (\{2, $x$\}, $x$) $26.21\%$\\
% \midrule
% \multirow{2}*{Smallest $C_W$} & (\{0, $x$\}, $x$) (\{1, $x$\}, $x$) (\{1, $x$\}, $x$) $38.94\%$ 
% \\

% ~ & (\{0, $x$\}, $x$) (\{1, $x$\}, $x$) (\{2, 2\}, $x$) $54.49\%$   \\

% \toprule Tasks (AUC) & Closure and Triangle \textit{v.s.} Wedge (57.58) \\
% \midrule
% \multirow{2}*{Largest $C_W$} & (\{0, $x$\}, $x$) (\{1, $x$\}, $x$) (\{2, $x$\}, 1) $84.26\%$\\

% ~ & (\{0, $x$\}, $x$) (\{1, $x$\}, $x$) (\{2, $x$\}, 2) $66.13\%$\\
% \midrule
% \multirow{2}*{Smallest $C_W$} & \bf{(\{0, $x$\}, $x$) (\{1, $x$\}, $x$) (\{1, $x$\}, $x$)} $34.68\%$ \\
% ~ & \bf{(\{$x$, 0\}, $x$) (\{$x$, 1\}, $x$) (\{$x$, 2\}, $x$)} $49.74\%$ \\


% \toprule Tasks (AUC) & Wedge \textit{v.s.} Edge (71.10)\\
% \midrule
% \multirow{2}*{Largest $C_W$} & (\{$x$, 0\}, $x$) (\{$x$, 1\}, $x$) (\{$x$, 2\}, 2) $49.14\%$\\
% ~ & (\{$x$, 0\}, $x$) (\{$x$, 1\}, $x$) (\{$x$, 2\}, $x$) $50.26\%$ 
% \\
% \midrule
% \multirow{2}*{Smallest $C_W$} & \bf{(\{$x$, 0\}, $x$) (\{$x$, 1\}, $x$) (\{1, 2\}, $x$)} $24.60\%$ \\
% ~ & \bf{(\{$x$, 0\}, $x$) (\{$x$, 1\}, $x$) (\{2, 2\}, $x$)} $28.81\%$ \\

% % ~ & (\{$x$, $x$\}, 0) (\{2, $x$\}, 1) (\{$x$, $x$\}, 2) $93.94\%$ & \bf{(\{$x$, $x$\}, 0) (\{$x$, $x$\}, 1) (\{$x$, $x$\}, 2)} $49.88\%$ & \bf{(\{0, $x$\}, $x$) (\{1, $x$\}, $x$) (\{2, 2\}, $x$)} $52.69\%$
% % \\
% \bottomrule 

% \caption{\small{TRWs with the top-2 largest and smallest scores $C_W$ (Eq.~\eqref{eq:TRW-score}) to distinguish two patterns in tags-ask-ubuntu. TRWs are categorized based on DEs: Given a node triplet $(\{u,v\},w,t)$, a TRW $W$ is categorized based on $W = I(W[0])\,I(W[1])\,I(W[2])$ where $I(a)=(\{\tilde{g}(a;S_u),\tilde{g}(a;S_v)\},\tilde{g}(a;S_w))$, where $\tilde{g}(a;S_z)$ uses SPD (Eq.\eqref{eq:spd}) and $x$ indicates SPD$\geq3$. \proj uses these TRWs and the decoder in Sec.~\ref{sec:decoder-3}. The ratio besides each TRW refers the number of the corresponding TRWs that appear as features for the first class over that for both classes.} \yunyu{Currently like this, maybe we can combine figure 7 and Table 5?}}\label{tab:interpretation}  
